Toward Learning Human-aligned Cross-domain Robust Models by Countering Misaligned Features

Machine learning has demonstrated remarkable prediction accuracy over i.i.d data, but the accuracy often drops when tested with data from another distribution. In this paper, we aim to offer another view of this problem in a perspective assuming the reason behind this accuracy drop is the reliance of models on the features that are not aligned well with how a data annotator considers similar across these two datasets. We refer to these features as misaligned features. We extend the conventional generalization error bound to a new one for this setup with the knowledge of how the misaligned features are associated with the label. Our analysis offers a set of techniques for this problem, and these techniques are naturally linked to many previous methods in robust machine learning literature. We also compared the empirical strength of these methods demonstrated the performance when these previous techniques are combined, with an implementation available at https://github.com/OoDBag/WR

==> secs/method.tex <==
%%%%%
% main message: the bound naturally leads sets of solutions of learning robust models, some of them have been proposed in many of different contexts, and also inspires a new one. 
% background: there are multiple existing methods, and they all require the knowledge of spurious features or the assumption of these features. 
%%%%%

We continue to study how our analytical results above can lead to 
practical methods to learn human-aligned robust models. 
We first show that our discussion
can naturally connect to existing methods for robust machine learning 
discussed in Section~\ref{sec:related}. 
Further, as these methods 
mostly require some prior knowledge of the misaligned features, 
we continue to explore a new method that does not require so. 

\subsection{Connections to Previous Robust Methods:}
Theorem~\ref{thm:cua} suggests that
training a human-aligned robust model amounts to training 
for small $c(h_\theta)$ and small empirical error (\textit{i.e.}, $\wepst$). 

\begin{comment}
\textbf{Connections to Distributionally Robust Optimization}

Choices are DRO $:=$ \{GroupDRO, CVaR, Reparemeterized DRO\}

In general, DRO considers a set of distribution that we want the model to perform well on in the uncertainty/perturbation set $\cal Q$.

\begin{equation}
    \min _{h_\theta \in \mathcal{H}} \max _{q \in \mathcal{Q}} \mathbb{E}_{(x, y) \in q}[\ell(x, y ; h_\theta)]
\end{equation}

In practice, we implement the DRO as GroupDRO using group meta data constructed from the identified aligned and misaligned features. Suppose the training distribution $\mP$ is assumed to be a mixture of two groups indexed by $\mathcal{G}=\{1,2\}$. So $\mathcal{Q} := \{ \mathbf{x}_{\mathcal{A}(f_{h},x)}, \mathbf{x}_{\mathcal{A}(f_{m},x)} \}$ %\{ \mathbf{x}_{\mathcal{A}(f_{m_i},x)} \}_{i=1}^g$

In this scenario, we replace the inner maximization as $\mathcal{R}(h_\theta)=\max_{g \in \mathcal{G}} \mathbb{E}_{(x, y) \sim P_{g}}[\ell(h_\theta ;(x, y))]$. So the overall problem becomes:

\begin{equation}
    \widehat{h_\theta}^{\text{DRO}}:=\underset{h_\theta \in \mathcal{H}}{\arg \min }\hat{\mathcal{R}}(h_\theta)
    % \left\{ :=\max _{g \in \mathcal{G}} \mathbb{E}_{(x, y) \sim \hat{P}_{g}}[\ell(h_\theta ;(x, y))]\right\}
\end{equation}

Intuitively, the DRO is a worst-case reweighting algorithm: GroupDRO in particular upweights the minority group based on protected attributes indicated by the the active set $\mathcal{A}(f_{m_i},x)$. 

\hl{Another DRO called CVaR: Define the uncertainty set $\mathcal{Q}$ as all samle distributions that are $\alpha$-covered by the training data. CVaR upweights groups incurring high losses and downweighting groups with low losses to ensure uniformly good performance across subpopulation and guarantees low losses on all $\alpha$-fraction subpopulations of the training distribution}
\end{comment}
\begin{comment}
Recall the dependency of $h_\theta$ on the active set of $f$ are described as
\begin{align}
    r(h_\theta, \mathcal{A}(f,\x)) = \max_{\x_{\mathcal{A}(f,\x)} \in \dom(f)_{\mathcal{A}(f,\x)}} |h_\theta(\x) - \y|,
    \label{eq:r}
\end{align}
And the definition of $c(h_\theta)$

\begin{align*}
c(h_\theta) = \dfrac{1}{n}\sum_{(\x, \y) \in (\X, \Y)_{\mP_s}} \mathbb{I}[h_\theta(\x)=\y]r(h_\theta, \mathcal{A}(\s,\x)).
\end{align*}

\begin{align*}
\tilde{c}(h_\theta) = \dfrac{1}{n}\sum_{(\x, \y) \in (\X, \Y)_{\mP_s}} \mathbb{I}[h_\theta(\x)\ne \y]r(h_\theta, \mathcal{A}(\s,\x)).
\end{align*}

define perturbation set $\cal Q$ as the samples the model fail on. %\hl{Connect with sample reweighting, Weighted Risk Minimization like (CVaR) GroupDRO, Unit DRO, LFF and JTT, Learning to Reweight Examples for Robust Deep Learning}
\end{comment}

\subsubsection{Connections to (Worst-case) Data Augmentation}
We can consider the upper bound of $c(h_\theta)$
\begin{align}
\begin{split}
    c(h_\theta) 
    \leq &\dfrac{1}{n}\sum_{(\x,\y)\in (\X,\Y)} r(h_\theta, \mathcal{A}(\s,\x)) \\
    = & \dfrac{1}{n}\sum_{(\x,\y)\in (\X,\Y)} \max_{\x_{\mathcal{A}(\s,\x)} \in \dom(\s)_{\mathcal{A}(\s,\x)}} |h_\theta(\x) - \y|,
    \label{eq:method:worst}
\end{split}
\end{align}
which intuitively means that 
instead of $c(h_\theta)$ that studies only the correct predictions because $h_\theta$ learns $\s$, 
now we study any predictions because $h_\theta$ learns $\s$. 

Further, as 
\begin{align*}
    |h_\theta(\x) - \y| \leq \max_{\x_{\mathcal{A}(\s,\x)} \in \dom(\s)_{\mathcal{A}(\s,\x)}} |h_\theta(\x) - \y|
\end{align*}
training for small $\eqref{eq:method:worst}$
naturally subsumes training for small empirical loss. 
Therefore, 
after we replace $|h_\theta(\x) - \y|$ with a generic loss term $\ell(h_\theta(\x),\y)$,
we can directly train a model with
\begin{align}
    \min_{h_\theta \in \mathcal{H}} \max_{\x_{\mathcal{A}(\s,\x)} \in \dom(\s)_{\mathcal{A}(\s,\x)}} \dfrac{1}{n}\sum_{(\x,\y)\in (\X,\Y)}  \ell(h_\theta(\x),\y)
    \label{eq:method:worst-da-result}
\end{align}
to get a model with small $c(h_\theta)$ and small empirical error. 

The above method is to augment the data by perturbing the misaligned features to maximize the training loss 
and solve the optimization problem with the augmented data. 
This method is the worst-case data augmentation method \citep{FawziSTF16} we discussed previously
and is closely connected to one of the most widely accepted methods 
for the adversarial robust problem, the adversarial training \citep{MadryMSTV18}.

While the above result shows that a method for learning human-aligned robust models is in mathematical connection to the worst-case data augmentation, 
in practice, a general application of this method will require some additional assumptions. 
The detailed discussions of these are in the appendix. 
\label{sec:worst-da}
\subsubsection{Connections to Distributionally Robust Optimization (DRO)}
We generalize the above analysis of worst-case data augmentation to a DRO problem \citep{ben2013robust, duchi2021statistics}. Given $n$ data points, consider a perturbation set $\mathcal{Q} := \{ \mathbf{x}_{\mathcal{A}(f_m, \mathbf{x}_i)} \in \operatorname{dom}(f)_{\mathcal{A}(f_m, \mathbf{x}_i)} \}_{i=1}^n$ encoding the features of $\x$ indexed by $\mathcal{A}(f,\x)$ over input space $\dom(f_m)$. Denote $q(\x, \y)$ and $p(\x,\y)$ are densities from the $\mathcal{Q}$ and training distribution $\mathcal{X} \times \mathcal{Y}$, respectively. Then (\ref{eq:method:worst-da-result}) can be rewritten as a DRO problem over a new distribution $\mathcal{Q}$.

\begin{equation}
    c(h_\theta) \le \min_{h_\theta \in \mathcal{H}} \max_{(\x_i,\y_i)\in \mathcal{Q}} \dfrac{1}{n}\sum_{i=1}^{n} \ell(h_\theta(\x_i),\y_i)
\end{equation}

$\mathcal{Q}$ encodes the priors about feature perturbation that model should be robust to. Therefore, choosing $f$-divergence as the distance metric where $f$ is convex with $f(1) = 0$, $\delta > 0$ as a radius to control the degree of the distribution shift, adversarial robustness in Section~\ref{sec:worst-da} can be viewed as an example of DRO on an infinite family of distributions with implicit assumptions that samples in $\mathcal{Q}$ are visually indistinguishable from original ones. For $p$ and $q$ that $p(\x, \y) = 0$ implies $q(\x, \y) = 0$, we arrive at a generic weighted risk minimization (WRM) formulation \citep{NIPS2016_4588e674, duchi2021statistics} when weights (by default as density ratios) $\lambda_\phi = q(\x, \y)/p(\x,\y)$ in (\ref{eq:method:wrm_loss}) derived from misaligned functions for 
\begin{align}
\begin{split}
    c(h_\theta) \le \min _{h_\theta \in \mathcal{H}} \max _{\lambda_\phi \in \mathcal{U}_f} \frac{1}{n} \sum_{i=1}^{n} \lambda_{\phi}\left(\x_{i}, \y_{i}\right) \cdot \ell\left(h_{\theta}\left(\x_{i}\right), \y_{i}\right)
    %\label{eq:method:wrm}
    \label{eq:method:wrm_loss}
\end{split}
\end{align}

where the uncertainty set $\mathcal{U}_f$ is reformulated as 
\begin{align}
%\begin{equation}
\mathcal{U}_f := \{\lambda_\phi(\x_i,\y_i)| & D_f(q(\x_i,\y_i)||p(\x_i,\y_i)) \le \delta, \\ & \sum_{i=1}^{n}\lambda_\phi(\x_i,\y_i)=1, \\ & \forall \lambda(x_i,y_i)\ge 0 \}
%\end{equation}
\end{align}

Intuitively, learner $\theta$ and adversary $\phi$ are playing a minimax game where $\phi$ finds worst-case weights and computationally-identifiable regions of errors to improve the robustness of the learner $h_\theta$. In this scenario, we unify a line of WRM approaches where weights $\lambda_\phi$ are mainly determined by misaligned features $\mathcal{A}(f_m, \mathbf{x})$, either parameterized by a biased model or derived from some heuristic statistics. 

%We consider an extended active sets $\tilde{\mathcal{A}}$ defined as
%\begin{equation}
%    \tilde{\mathcal{A}} = (\mathop{\cup}\limits_{i=1}^{n} \mathcal{A}(f_m,\mathbf{x}_i) ) \bigcup (\mathop{\cup}\limits_{j=1}^{n} \mathcal{A}(f_h,\mathbf{x}_j) )
%\end{equation}
\begin{comment}
Following Eq. (\ref{eq:method:worst-da-result})
\begin{align}
\begin{split}
    c(h_\theta) 
    & \leq \min_{h_\theta \in \mathcal{H}} \max_{\mathbf{x}_{\tilde{\mathcal{A}}}} 
    \dfrac{1}{n}\sum_{i=1}^{n}  \ell(h_\theta(\x_i),\y_i) \\ & = 
    \min_{h_\theta \in \mathcal{H}} \dfrac{1}{n}\sum_{i=1}^{n}  \ell(\frac{w_{i} h_\theta(\x_{i})}{\sum w_{i}},\y_i) \\ & 
    \leq \min_{h_\theta \in \mathcal{H}} \dfrac{1}{n} \frac{w_{i} \ell(h_\theta(\x_i),\y_i)}{\sum w_{i}} \\ &
    \leq \min_{h_\theta \in \mathcal{H}} \dfrac{\lambda_m}{n} \sum_{i=1}^{n} \ell(h_\theta(\x_i),\y_i)
    \label{eq:method:wrm_loss}
    % (\x,\y)\in (\X,\Y) 
\end{split}
\end{align}
\end{comment}
%Adversarial WRM with f-divergence. \hl{Worst-case parameterization or simply assigns larger weight $w_i$ to data $(x_i, y_i)$ with a larger loss.}
% where $\lambda_m \ge 1$ is a constant and $w_i$ is a sample-wise weight such that $\lambda_\phi$ in (\ref{eq:method:wrm}) is converted as $w_i/\sum w_i$ with various design choices.

%The first inequality extends the features by the union of active sets. The second equality follows the assumption that the training data can be approximated by the mixture of other data points, normalized by the sum of weights. Intuitively, the assumption shows that searching the worst-case sample over misaligned and aligned feature spaces are equivalent to WRM, which is a common practice when data contains meta information about subpopulation under mild conditions \citep{rockafellar2000optimization, duchi2020distributionally, Sagawa*2020Distributionally}. Here we consider the most generic case where covariates are form by mixing any pair of data points from raw dataset\footnote{can also be seen as treating each data point as a subpopulation}. By the convexity of cross-entropy and Jensen inequality, we arrive at the third inequality. Then for variants of WRM methods, differences are only the determined of mixing coefficients $w_i$ or $\lambda_m$. Therefore, the learning via WRM is essentially minimizing the upper bound of $c(h_\theta)$.

\begin{comment}
\begin{align}
\begin{split}
    c(h_\theta) 
    & \leq \lambda_{m} c(h_\theta) + \lambda_{h} \tilde{c}(h_\theta) \\ & = \dfrac{\lambda_{m}}{n}\sum_{(\x,\y)\in (\X,\Y)_{\mP_s}} \mathbb{I}[h_\theta(\x)= \y] r(h_\theta, \mathcal{A}(\s,\x)) \\ & + \dfrac{\lambda_h}{n}\sum_{(\x, \y) \in (\X, \Y)_{\mP_s}} \mathbb{I}[h_\theta(\x)\ne \y]r(h_\theta, \mathcal{A}(\s,\x)) \\
    \label{eq:method:generic}
\end{split}
\end{align}
\end{comment}

On one hand, for those $\phi$ is parameterized as a second player, we consider the following two approaches:

\textbf{Adversarially reweighted learning (ARL) \citep{NEURIPS2020_07fc15c9}} is a variant of DRO that uses an adversary model $f_\phi$ (for a slight abuse of notation) to identify samples with misaligned features and regions where the learner makes significant errors. Similar to (\ref{eq:method:wrm_loss}), it learns worst-case per-example importance weights for training $h_\theta$ via minimizing the upper bound of $c(h_\theta)$, where $\lambda_{\phi}\left(\x_{i}, \y_{i}\right)=1+n \cdot \frac{f_{\phi}\left(\x_{i}, \y_{i}\right)}{\sum_{i=1}^{n} f_{\phi}\left(\x_{i}, \y_{i}\right)}$. Note that we only consider the first iteration of ARL and it is straightforward to extend the analysis to an iterative version.

\textbf{Learning from failures (LFF) \citep{nam2020learning}} trains a biased neural network $h_\phi$ by amplifying its early-stage predictions and a debiased neural network $h_\theta$ by focusing on samples that the biased model struggles to learn.Then re-weight training samples using the relative difficulty score based on the loss of the biased model and the debiased model. Assuming $h_\theta$ and $h_\phi$ are from the same hypothesis space $\mathcal{H}$, we have $h_\phi$ trained by the generalized cross entropy loss as 

\begin{align}
\begin{split}
    \min_{h_\phi \in \mathcal{H}} \frac{1}{n} \sum_{i=1}^{n} \ell_{\operatorname{gce}}\left(h_\phi(\x_i), \y_i\right)
    \label{eq:method:lff_biased} 
\end{split}
\end{align}

LFF serves as a special case of (\ref{eq:method:wrm_loss}) that $h_\theta$ is learned by optimizing (\ref{eq:method:wrm_loss}) when $\lambda_\phi(\x_i,\y_i)=\frac{\ell_{\operatorname{ce}}\left(h_\phi(\x_i), \y_i\right)}{\ell_{ce}\left(h_\phi(\x_i), \y_i\right)+\ell\left(h_\theta(\x_i), \y_i\right)}$ is the weighted average of the cross entropy prediction of $h_\phi$ and $h_\theta$.

\begin{comment}
\begin{align}
\begin{split}
    c(h_\theta) \le \min_{h_\theta \in \mathcal{H}} \frac{1}{n} \sum_{i=1}^{n} \mathcal{W}(\x_i) \cdot \ell \left(h_\theta(\x_i), \y_i\right) \label{eq:method:lff_debiased} 
\end{split}
\end{align}

where \begin{align}
\begin{split}
\mathcal{W}(x)=\frac{\ell_{\operatorname{ce}}\left(h_\phi(\x_i), \y_i\right)}{\ell_{ce}\left(h_\phi(\x_i), \y_i\right)+\ell\left(h_\theta(\x_i), \y_i\right)}
\label{eq:method:lff_weight}
\end{split}
\end{align}
\end{comment}

On the other hand, in the following special cases, $\phi$ is a constant chosen by some approximate solutions or heuristics.

\textbf{DRO with structural assumptions \citep{hu2018does}} takes a perspective that the training distribution is a mixture of multiple groups such that the perturbation set $\mathcal{Q}$ is composed of any mixture of these groups. % KL-DRO \citep{hu2013kullback}, and Conditional value at risk (CVaR) \citep{rockafellar2000optimization}. encoding a pre-determined family of distributions or parametric generative models

We consider the GroupDRO \citep{Sagawa*2020Distributionally} variant, which assumes data can be grouped by available meta-information such as demographics. Intuitively, data within the group are likely to share the same distribution. Defining the perturbation set according to group labels or demographic attributes, GroupDRO re-samples the training data for learning model parameters according to the worst group loss.
% and CVaR or the average of the $\lceil \alpha N\rceil$ ($\alpha \in [0,1]$, N is the amount of population) largest. , respectively.
\begin{align}
\begin{split}
c(h_\theta) \le \min_{h_\theta \in \mathcal{H}} \frac{1}{n} \sum_{g=1}^{m} \lambda_{g} \sum_{i=1}^{|P_{g}|}\ell(h_\theta ;(\x_i, \y_i))
\end{split}
\end{align}
where $P_g$ is indexed by $m$ groups forming the entire dataset as $\mathcal{P}=\left\{P_{g}\right\}_{g=1}^{|\mathcal{P}|}$. In practice, $\lambda_g$ is determined by $\exp \left(\ell\left(h_{\theta}(\x_i), \y_i)\right)\right)/ \sum\limits_{j=1}^{n} \exp \left(\ell\left(h_\theta(\x_j), \y_j)\right)\right)$ for any $(\x_i, \y_i) \in P_g$. Since samples within the same group are assigned weights homogeneously, obviously it is a special case of (\ref{eq:method:wrm_loss}).

%KL-DRO shows worst-case expectation admits an analytically tractable solution and can be levaeraged to convert KL constrained DRO into per-sample WRM problem, which is essentially optimizing the (\ref{eq:method:wrm_loss}) objective.

\textbf{Just train twice (JTT) \citep{pmlr-v139-liu21f}} works in a case where failure samples from ERM are resampled to form a two-group optimization problem. Intuitively, JTT upweights the identified failure samples (denoted as $\mathcal{D}_{f}$) with misaligned features $\lambda_{up}$ times and retrain the model for a second time by essentially optimizing the upper bound of $c(h_\theta)$ in (\ref{eq:method:wrm_loss}) where $\lambda_\phi$ are set to be $(\lambda_{up}+1)$ for failure samples and $1$ for correctly predicted samples in the first round

%\begin{comment}
\begin{align}
\begin{split}
    c(h_\theta) 
    & \leq \min _{h_\theta \in \mathcal{H}} \frac{1}{n} \sum_{i=1}^{n} (\lambda_{up}[\mathbbm{1}[(\x_i,\y_i) \in \mathcal{D}_{f}]]+1)  \ell\left(h_{\theta}\left(\x_{i}\right), \y_{i}\right)
    %c(h_\theta) + \tilde{c}(h_\theta)
    \label{eq:method:jtt}
\end{split}
\end{align}
%\end{comment}

\subsubsection{Connections to Regularizing the Hypothesis Space}
Connecting our theory to the other main thread is little bit tricky, 
as we need to extend the model to an encoder/decoder structure, where we use $E_\theta$ and $D_\theta$ to denote the encoder and decoder respectively. 
Thus, by definition, we have $h_\theta(\x) = D_\theta(E_\theta(\x))$.  
Further,
we define $\s'$ as the equivalent of $\s$ with the only difference is that 
$\s'$ operates
on the representations $E_\theta(\x)$. 
With the setup, 
optimizing the empirical loss and $c(h_\theta)$ leads to (details in the appendix):
\begin{align}
    \min_{D_\theta, E_\theta}\dfrac{1}{n}\sum_{(\x,\y)\in (\X,\Y)}\ell(D_\theta(E_\theta(\x)), \y) - \ell(\s'(E_\theta(\x)), \y), 
    \label{eq:regularization}
\end{align}
which is highly related to methods used to learn auxiliary-annotation-invariant representations, 
and the most popular example of these methods is probably DANN \citep{GaninUAGLLML16}. 

Then, the question left is how to get $\s'$. 
We can design a specific architecture given the prior knowledge of the data, then $\s'$ can be directly estimated through
\begin{align*}
    \min_{\s'} \dfrac{1}{n}\sum_{(\x,\y)\in (\X,\Y)} \ell(\s'(E_\theta(\x)),\y), 
\end{align*}
which connects to several methods in Section~\ref{sec:related}, such as \citep{WangGLX19, bahng2019learning}. 
Alternatively, we can estimate $\s'$ with additional annotations (\textit{e.g.}, domain ids, batch ids \textit{etc}), then we can estimate the model by (with $\mathbf{t}$ denoting the additional annotation) 
\begin{align*}
    \min_{\s'} \dfrac{1}{n}\sum_{(\x,\mathbf{t})\in (\X,\mathbf{T})} \ell(\s'(E_\theta(\x)),\mathbf{t}),
\end{align*}
which connects to methods in domain adaptation literature such as \citep{GaninUAGLLML16,li2018domain}. 

%%% Discussion of the connection (to put in the appendix) %%% 


% In this section, 
% we will take advantage 
% of our analysis to introduce 
% methods that can be used to learn robust models 
% by countering the spurious correlation. 
% First, we discuss the 
% principled solutions that can 
% lead to the error bound in Theorem~\ref{thm:cua} to be smaller. 
% These methods are interestingly linked to 
% many previously established methods in robustness in general. 
% Second, 
% as all above methods will require 
% some knowledge of $\s$ or $\mathcal{A}(\s,\x)$, 
% we also explore a new method 
% that does not require so. 


% \textbf{Data augmentation}
% Alternatively, we can assume 
% \begin{align}
%     \mathbb{E}_{\x_{\mathcal{A}(\s,\x)} \sim \mathbf{P}^{\textnormal{all}}_{\mathcal{A}(\s,\x)}} |h_\theta(\x) - \y| = \max_{\x_{\mathcal{A}(\s,\x)} \in \mathcal{X}_{\mathcal{A}(\s,\x)}} |h_\theta(\x) - \y|,
% \end{align}
% where $\mathbf{P}^{\textnormal{all}}$ denotes the distribution that 
% can help to remove the correlation 
% between $\s$ related features and $\y$ 
% (\textit{e.g.}, a uniform distribution 
% over $\mathcal{X}$ is sufficient, 
% but $\mP_s$ 
% will not be good enough). 
% The main strategy is to train with
% the samples whose $\s$ related features are randomized, so that the model 
% is expected to learn to ignore the pattern. 
% As $\x$ can usually be sampled by $\mathbf{P}^{\textnormal{all}}$, 
% one can drop the generic loss and train a model with
% \begin{align}
%     \min_h_\theta \dfrac{1}{n}\sum_{(\x,\y)\in (\X,\Y)} \mathbb{E}_{\x_{\mathcal{A}(\s,\x)} \sim \mathbf{P}^{\textnormal{all}}_{\mathcal{A}(\s,\x)}} l(h_\theta(\x),\y). 
% \end{align}


% One can also use consistency loss to foster the invariance learning of the undesired patterns \citep{ourwork}. 

% We can also consider to find a $\cal H_{\textnormal{regularized}}$ so that
% \begin{align}
%     |h_\theta(\x) - \y| = \max_{\x_{\mathcal{A}(\s,\x)} \in \mathcal{X}_{\mathcal{A}(\s,\x)}} |h_\theta(\x) - \y| \quad \textnormal{for} \quad h_\theta \in \mathcal{H}_{\textnormal{regularized}}, 
% \end{align}
% which intuitively means that 
% for any $h_\theta \in \cal H_{\textnormal{regularized}}$, $h_\theta$ ignores the information from $\mathcal{A}(\s,\x)$. 
% There is a proliferation of recent developments of this thread, 
% either through 
% intuitive understanding of the task 
% or the data \citep[\textit{e.g.},][]{WangGLX19,WangHLX19,bahng2019learning}
% or through theoretical understanding
% for rigorously defined perturbations \citep[\textit{e.g.},][]{abadeh2015distributionally,cranko2020generalised}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% details to put in appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Before we connect these methods, we need two more assumptions:
% \begin{itemize}
%     \item [\textbf{A5}:] \textbf{Separation of Features:} 
%     For any $\x \in \mathcal{X}$, $\mathcal{A}(\h,\x) \cap \mathcal{A}(\s,\x) = \emptyset$
%     \item [\textbf{A6}:] \textbf{Separation of Functions:}
%     For any $\x \in \mathcal{X}$ and $\s$, 
%     there exists a subspace $\dom(\x, \s) \subseteq \mathcal{X}$ as a function of $\x$ and $\s$, where 
%     \begin{align*}
%         \min_{\x \in \dom(\x, \s)}|\h(\x)-\y|=|\h(\x)-\y|
%     \end{align*}
% \end{itemize}
% These two assumptions regularize the behaviors the functions 
% in the sense that ``perturbations of the features used by one function will not alter the prediction of the other''. 
% Although these assumptions appear strong, 
% we argue these assumptions are essential for a general discussion 
% of methods that can work in practice. 
% For example, 
% in image classification, 
% the image background sometimes is a spurious feature, 
% which is separable from the object the image depicts;
% as another example, 
% in text classification, 
% the spurious features can be some keywords, 
% which are part of the features used 
% by the desired function to understand the semantics of the sentences:
% these keywords can usually not be replaced with an arbitrary word, but only with its own synonyms. 

% We extend the model to a encoder/decoder structure, where we use $h_\theta_e$ and $h_\theta_d$ to denote the encoder and decoder respectively. By definition, we have $h_\theta(\x) = h_\theta_d(h_\theta_e(\x))$, and we use $\e=h_\theta_e(\x)$. 
% With the encoder/decoder structure, we define $\s'$ as the misaligned function that operates on the representations. 

% Sometimes $\s'$ requires a specific design of the architecture given the prior knowledge of the data, then $\s'$ can be directly estimated through 
% \begin{align*}
%     &\min_{\s'} \dfrac{1}{n}\sum_{(\x,\y)\in (\X,\Y)} l(\s'(h_\theta_e(\x)),\y)
% \end{align*}
% If there is no specially designed architecture involved, then the estimation of $\s'$ needed to be guided by other labels (\textit{e.g.}, domain ids, batch ids \textit{etc}.), then we have
% \begin{align*}
%     &\min_{\s'} \dfrac{1}{n}\sum_{(\x,\mathbf{t})\in (\X,\mathbf{T})} l(\s'(h_\theta_e(\x)),\mathbf{t})
% \end{align*}
  

% \begin{algorithm}[H]
% \small 
% \SetAlgoLined
% \KwResult{$h_\theta^T$}
% \textbf{Input:} $T$, $\rho$, $(\X,\Y)$\; 
%  initialize $h_\theta^{(0)}$, $t=1$, $\eta$, $\tau$\;
%  \While{$t \leq T$}{
%  \For {sample $(\x,\y)$}{
%     update $h_\theta_e^{(t)}$ with standard gradient descent\;
%     calculate $\e=h_\theta_e^{(t)}(\x)$\;
%     calculate the gradient $\mathbf{g} = \partial l(h_\theta_d^{(t-1)}, \e, \y)/\partial\e$\;
%     set the threshold $\tau(\rho, \mathbf{g})$ 
%     %to be the $\rho$\textsuperscript{th} quantile of $|\mathbf{g}|$ 
%     and set $\mathcal{A}(h_\theta^{(t-1)}, \e) = \{i | \vert\mathbf{g}_i\vert \geq \tau(\rho, \mathbf{g})\}$\;
%     sample $\z = \e_{\mathcal{A}(h_\theta_d^{(t-1)}, \e)} + \tau (\partial l(h_\theta^{(t-1)}, \e, \y)/\partial\e)_{\mathcal{A}(h_\theta_d^{(t-1)}, \e)}$\;
%     calculate the gradient $\mathbf{g}' = \partial l(h_\theta^{(t-1)}, \z, \y)/\partialh_\theta_d^{(t-1)}$\;
%     update the model $h_\theta_d^{(t)} = h_\theta_d^{(t-1)} - \eta\mathbf{g}'$
%  }
%  }
%  \caption{Learning Robust Models with Minimum Supervision}
%  \label{algorithm:main}
% \end{algorithm}  

% \subsection{Learning Robust Models with Minimum Supervision}
% While our formal study suggests that 
% we cannot have a human-aligned model without the knowledge of $\s$ or $\h$, 
% we continue to ask 
% what the best we can do empirically without such knowledge, inspired by the analysis. 
% Now, we consider another upper bound of $c(h_\theta)$: 
% if we use $\mathcal{F}$ to denote the set $\{\h, \s\}$ and use $i$ to index the element of $\mathcal{F}$, we can have the following upper bound to optimize
% \begin{align}
%     c(h_\theta) 
%     %=  \dfrac{1}{n}\sum_\x \mathbb{I}[h_\theta(\x)=\y]r(h_\theta, \mathcal{A}_\mP(f_b,\x)) 
%     \leq \dfrac{1}{n}\sum_{(\x,\y) \in (\X,\Y)} r(h_\theta, \mathcal{A}(\s,\x))
%     \leq \dfrac{1}{n}\sum_{(\x,\y) \in (\X,\Y)}\sum_i r(h_\theta, \mathcal{A}(\mathcal{F}_i,\x)).
%     \label{eq:ms}
% \end{align}

% By optimizing the RHS of \eqref{eq:ms}, we aim to discourage the learning towards functions that 
% \emph{only} rely on one labeling function for each sample for \emph{any} labeling functions. 
% Intuitively, the method is to encourage the 
% model's usage in \emph{all} possible features (either associated with $\h$ or $\s$); 
% thus, the model may be more robust to the changes of features 
% when dealing with perturbations of the data. 

% A method using all the features is not expected to be better 
% than a method that only uses the $\h$ associated features. 
% However, as many other methods
% require specific knowledge of the misaligned features, 
% we believe this method is a better practice 
% than vanilla training \eqref{eq:train}
% when there is no side information
% about either $\h$ or $\s$, 
% since we can probably use the model estimated in the previous iteration 
% as a substitute of $\h$ or $\s$. 
% This substitution is an intuitive extension of Assumption \textbf{A3}, 
% which suggests that a model will learn either $\h$ or $\s$ 
% if it can predict the sample correctly. 

% Therefore, a single iteration of our proposed algorithm can be sketched as the follows: At iteration $t$
% \begin{itemize}
%     %\item Use $h_\theta^{(t-1)}$ as a substitute of either $\h$ or $\s$. 
%     \item Identify $\mathcal{A}(h_\theta^{(t-1)}, \x)$ according to \eqref{eq:a:def}
%     \item Sample $\z = \argmax_{\x_{\mathcal{A}(h_\theta^{(t-1)}, \x)} \in \dom(h_\theta^{(t-1)})_{\mathcal{A}(h_\theta^{(t-1)}, \x)}}|h_\theta^{(t-1)}(\x)-\y|$
%     \item Continue to train the model with $\z$ to get $h_\theta^{(t)}$
% \end{itemize}
% where the second step is the worst-case data augmentation. 

% Further, this idea can be straightforwardly extended to the encoder/decoder structure 
% following the related discussion in the previous section. 
% With $h_\theta_e$ and $h_\theta_d$ denoting the encoder and decoder respectively and $\e = h_\theta_e(\x)$, 
% we have the algorithm sketched for the encoder/decoder structure as 
% \begin{itemize}
%     %\item Use $h_\theta^{(t-1)}$ as a substitute of either $\h$ or $\s$. 
%     \item Train the model in a standard manner to get $h_\theta_e$ and $\e = h_\theta_e(\x)$. 
%     \item Identify $\mathcal{A}(h_\theta_d^{(t-1)}, \e)$ according to \eqref{eq:a:def}
%     \item Sample $\z = \argmax_{\e_{\mathcal{A}(h_\theta_d^{(t-1)}, \e)} \in \dom(h_\theta_d^{(t-1)})_{\mathcal{A}(h_\theta_d^{(t-1)}, \e)}}|h_\theta_d^{(t-1)}(\e)-\y|$
%     \item Continue to train the decoder with $\z$ to get $h_\theta_d^{(t)}$
% \end{itemize}

% However, there are still challenges of the computational load to identify $\mathcal{A}(h_\theta_d^{(t-1)}, \x)$. 
% Interestingly, in the regime of the encoder/decoder structure, we notice that 
% our proposed method is quite similar to \cite{huang2020selfchallenging}, 
% which also follows a three-step procedure:
% 1) identify the features used by $h_\theta_d^{(t-1)}$ by checking the gradient
% 2) mask the identified features to be zeros
% 3) continue to train the model with the masked features. 
% Thus, we borrow the first step of \cite{huang2020selfchallenging} 
% to circumvent the computational load of identification of $\mathcal{A}(h_\theta_d^{(t-1)}, \x)$. 
% This also allows us to directly build our method upon the implementation of \cite{huang2020selfchallenging}. 
% % {\color{blue}
% % Also, directly building our method upon the implementation of \cite{huang2020selfchallenging} 
% % also offers us a convenient way to show the advantages of our theoretical discussion 
% % because the only difference of our method in comparison to \cite{huang2020selfchallenging}
% % is the second step. According to our derivation, worst-case augmentation is a better second step than masking identified features to be zeros.}

% Further, we also use some heuristics to accelerate the augmentation. 
% Inspired by the fast gradient sign method \citep{goodfellow2015explaining}, 
% we sampled the embeddings that can lead to a worse loss by 
% $\z = \e_{\mathcal{A}(h_\theta_d^{(t-1)}, \e)} + \tau (\partial l(h_\theta^{(t-1)}, \e, \y)/\partial\e)_{\mathcal{A}(h_\theta_d^{(t-1)}, \e)}$, where $\tau$ is a scalar hyperparameter. 

% In summary, our analysis suggests that we can improve upon \cite{huang2020selfchallenging} to get a new algorithm with one major difference: 
% instead of masking identified embeddings to be zeros, 
% we sample the identified embeddings to ones that lead to a worse loss. 
% The algorithm is summarized in Algorithm~\ref{algorithm:main}. 



% % In practice, 
% % as we do not have the knowledge of $\mathcal{F}$, 
% % we can use the estimated $h_\theta$
% % from previous iteration as a substitute, 
% % also as the searching for $\mathcal{A}(f, \x)$ 
% % can be computationally expensive, 
% % we use the gradient information to 
% % guide the selection of the features. 
% % In summary, 
% % this new method, 
% % which we name \emph{minimum supervision (MS)}, 
% % has the following three major steps at iteration $t$:
% % \begin{itemize}
% %     \item Use $h_\theta^{(t-1)}$ as a substitute of either $\h$ or $\s$. 
% %     \item Identify $\mathcal{A}(h_\theta^{(t-1)}, \x)$ 
% % with top $\rho$ fraction of features according to the gradient.
% %     \item Sample $\x_{\mathcal{A}(h_\theta^{(t-1)}, \x)}$ over $\mathcal{X}_{\mathcal{A}(h_\theta^{(t-1)}, \x)}$ and continue to train the model. 
% % \end{itemize}
% % Thus, the new method has a hyperparameter $\rho$. 

% % In practice, 
% % as we do not have the knowledge of 
% % either $\h$ or $\s$ ($\mathcal{F}$), 
% % the strategy we use is to estimate the model first
% % and consider our estimated model $\wt$ 
% % as a substitute of the 
% % labeling function (either $\h$ or $\s$). 
% % Therefore, at each iteration $t$, 
% % we will use the $\wt$ at the previous 
% % iteration to identify the active set 
% % for the optimization of $\eqref{eq:ms}$ (in main manuscript). 

% % Further, another question is 
% % that when we have 
% % $\wt^{(t-1)}$, 
% % how to identify $\mathcal{A}(\wt^{(t-1)}, \x)$, 
% % as searching for $\mathcal{A}(\wt^{(t-1)}, \x)$ 
% % by the definition can be computationally expensive. 
% % Our practical strategy is to use the 
% % gradient of $\wt^{(t-1)}$ to  
% % guide the selection of the features. 
% % Intuitively, 
% % we argue that the 
% % the features with 
% % larger absolute values 
% % of $\partial l(h_\theta^{(t-1)}, \x, \y)/\partialh_\theta^{(t-1)}$
% % are the features 
% % $\wt^{(t-1)}$ relies on. 

% % Finally, 
% % we consider the 
% % features with 
% % values greater than a threshold $\tau(\rho, \mathbf{g})\}$ 
% % are the features that are in $\mathcal{A}(\wt^{(t-1)}, \x)$. 
% % The threshold hold is set as the $\rho$\textsuperscript{th} 
% % quantile of all the calculated gradients for this sample. 
% % The algorithm is shown in Algorithm~\ref{algorithm:main}

% % \begin{algorithm}[H]
% % \SetAlgoLined
% % \KwResult{$h_\theta^T$}
% % \textbf{Input:} $T$, $\rho$, $(\X,\Y)$\; 
% %  initialize $h_\theta^0$, $t=1$, $\eta$\;
% %  \While{$t \leq T$}{
% %  \For {sample $(\x,\y)$}{
% %     calculate the gradient $\mathbf{g} = \partial l(h_\theta^{(t-1)}, \x, \y)/\partialh_\theta^{(t-1)}$\;
% %     set the threshold $\tau(\rho, \mathbf{g})$ to be 
% %     the $\rho$\textsuperscript{th} quantile of $|\mathbf{g}|$\;
% %     set $\mathcal{A}(h_\theta^{(t-1)}, \x) = \{i | \vert\mathbf{g}_i\vert \geq \tau(\rho, \mathbf{g})\}$\;
% %     sample $\x'$ where $\x'_{\mathcal{A}(h_\theta^{(t-1)}, \x)} \in \mathcal{X}_{\mathcal{A}(h_\theta^{(t-1)}, \x)}$\;
% %     calculate the gradient $\mathbf{g}' = \partial l(h_\theta^{(t-1)}, \x', \y)/\partialh_\theta^{(t-1)}$\;
% %     update the model $h_\theta^t = h_\theta^{(t-1)} - \eta\mathbf{g}'$
% %  }
% %  }
% %  \caption{Learning Robust Models with Minimum Supervision}
% %  \label{algorithm:main}
% % \end{algorithm}

==> secs/related.tex <==

There is a rich history of 
learning robust models. 
We first discuss works in three topics, 
all centering around the concept of invariance, 
where invariance intuitively means the model's prediction 
preserves under certain shift of the data. 
We then highlight works related to our 
theoretical discussion. 

\textbf{Cross-domain Generalization}
This line of works probably originates from 
\emph{domain adaptation} \citep{ben2007analysis}, 
which studies the problem of 
training a model over one distribution 
and test it over another one.
Since \citep{GaninUAGLLML16}, 
recent advances along this topic 
mainly center around the concept of 
invariance: 
most techniques leverage different regularizers 
to learn representations that are invariant to the marginals of these two distributions \citep[\textit{e.g.},][]{ghifary2016deep,rozantsev2018beyond}. 
Further, the community aims beyond the situation 
that a trained model from domain adaptation may only be applicable 
to one distribution, 
and focuses on \emph{domain generalization} \citep{muandet2013domain}, 
which studies the problem of training 
a model over a collection of distributions 
and test it with distributions unseen during training. 
Similarly, most recent methods aim to learn representations 
invariant to the marginals of the training distributions \citep[\textit{e.g.},][]{motiian2017unified,li2018domain,carlucci2018agnostic}. 
Recently, 
the community extends the study to 
\emph{domain generalization without domain IDs} to 
address the real-world situations that 
domain IDs are unavailable
\citep{WangHLX19}, 
which again focuses on learning representations 
invariant to specifically designed functions. 

\textbf{Adversarially Robust Models}
The study of robustness against adversarial examples was popularized 
by the empirical observations that small perturbations on image data 
can significantly alter the model's prediction \citep{szegedy2013intriguing,goodfellow2015explaining}. 
This observation initiated a line of works 
building models 
invariant to such small perturbations 
(the rigorous definitions 
of ``small perturbations''
will not be discussed in details here) \citep[\textit{e.g.},][]{lee2017generative,akhtar2018defense}
and adversarial training \citep{MadryMSTV18} is currently the most widely-accepted method in terms of empirical defense. 
On the other hand, 
the community also aims to develop methods that 
are provably robust to predefined perturbations \citep[\textit{e.g.},][]{wong2018provable,Croce2020Provable}, 
which links back to the 
works of distributional robust models \citep[\textit{e.g.},][]{abadeh2015distributionally,Sagawa2020Distributionally}, 
whose central goal is to train models 
invariant to a predefined shift of distributions. 
Recent evidence shows key challenges of learning
adversarially robust models are spuriously correlated features \citep{ilyas2019adversarial, wang2020high}, 
connecting adversarial robustness to the next topic.  

\textbf{Countering Spurious Correlation}
Works along this line usually connects the robustness of a model 
to its ability of ignoring the spurious correlation in the data, 
which was also studied 
under the terminologies of \emph{confounding factors},
or \emph{dataset bias}. 
With different concrete definitions of the spurious correlation, 
methods have been developed for various applications, 
such as image/video classification 
\citep[\textit{e.g.},][]{goyal2017making,
%WangMMX17,
WangGLX19,WangHLX19, bahng2019learning,shi2020informative}, 
text classification \citep[\textit{e.g.},][]{he2019unlearn,clark2019don,bras2020adversarial,zhou2020towards,ko2020look}, 
medical diagnosis \citep[\textit{e.g.},][]{zech2018confounding,chaibub2019permutation, larrazabal2020gender} \textit{etc}. 
The key concept is, as expected, 
to be invariant to the spurious correlated features. 

\textbf{Related Theoretical Discussion}
Out of a rich collection of theoretical discussions in learning robust models, 
we only focus on the ones for 
\emph{unsupervised domain adaptation}, 
as they will be related to our discussions in the sequel.
Popularized by \citep{ben2007analysis,ben2010theory}, 
these analyses, 
although in various forms 
\citep{MansourMR09,GermainHLM16,ZhangLLJ19,dhouib2020margin}, 
mostly involve two additional terms than standard machine learning generalization bound: 
one term describes the ``learnable'' nature of the problem 
and one term quantifies the differences of the two distributions. 
This second term probably inspired 
most of the empirical methods forcing invariant representations 
from distributions. 
However, the value of invariance 
is recently challenged \citep{wu2019domain,ZCZG19}.
For example, \citet{ZCZG19} argued that 
``invariance is not sufficient'' 
by showing counter examples violating the ``learnable'' nature of the problem and formalized the understanding 
as that the two distributions have possibly different 
labeling functions. 
% which is linked to some empirical observations 
% (\textit{e.g.}, the failure of digit classification from MNIST to SVHN after invariance is forced \citep{GaninUAGLLML16}).  

\textbf{Key Difference:} 
However, we find the argument of disparity in labeling functions 
less intuitive, 
because human will nonetheless be able to 
agree on the label of an object
whichever distribution the object lies in:  
in the context of this paper,
we argue a shared labeling function always exists
(in any task reasonable to human), 
but the ERM model may not have
the incentive to learn this function 
and learns a spurious one instead. 
As in Figure~\ref{fig:intro}, 
we formalize the problem as learning against spurious functions, 
and argue that the central problem 
is still invariance, 
but instead of invariance to marginals, 
we urge for invariance to the spurious function. 
Our discussion also applies to more than 
unsupervised domain adaptation and 
relates to most of the topics discussed in this section. 
